Extended URDF: Accounting for parallel mechanism in robot description

Robotic designs played an important role in recent advances by providing powerful robots with complex mechanics. Many recent systems rely on parallel actuation to provide lighter limbs and allow more complex motion. However, these emerging architectures fall outside the scope of most used description formats, leading to difficulties when designing, storing, and sharing the models of these systems. This paper introduces an extension to the widely used Unified Robot Description Format (URDF) to support closed-loop kinematic structures. Our approach relies on augmenting URDF with minimal additional information to allow more efficient modeling of complex robotic systems while maintaining compatibility with existing design and simulation frameworks. This method sets the basic requirement for a description format to handle parallel mechanisms efficiently. We demonstrate the applicability of our approach by providing an open-source collection of parallel robots, along with tools for generating and parsing this extended description format. The proposed extension simplifies robot modeling, reduces redundancy, and improves usability for advanced robotic applications.

==> tex/4.Robot.tex <==
\section{Examples of Robots Models} \label{sec:toolbox}

To demonstrate the generality of the method, we provide a collection of robots with closed kinematics chains, described using our extended URDF format. The URDF are generated using Onshape to robot \cite{onshape2robot}, and the YAML file is either manually written or generated using a naming convention. We present the following models of the robots Digit and Kangaroo.

\subsection{Digit}
Digit is a humanoid robot designed to work in a factory, demonstrating locomotion capabilities while carrying boxes. Our work limited our modeling to the leg, as the upper body is purely serial and can be included in the standard URDF.
\begin{figure}[t!]
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=0.3\textwidth, trim={3cm 1cm 2cm 0cm}, clip]{Images/digit.png}
         \caption{Digit Robot}
         \label{fig:digitRobot}
     \end{subfigure}
     \hspace{0cm}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=0.32\textwidth, trim={3cm 1.5cm 3cm 5cm}, clip]{Images/digit_modeled.png}
         \caption{Modeled digit robot}
         \label{fig:digitModel}
     \end{subfigure}
    \caption{Digit real and modeled robot. In the model, the 6D contacts constraints are "opened" for better visualization}
    \label{fig:digit}
\end{figure}
The real and modeled robots are presented in Fig.~\ref{fig:digit}.
Digit's leg has 6 motors for 6 degrees of freedom (DoF). One can observe three kinematic closures per leg - one allows motion of the knee using a motor located in the hips, and two allows moving the ankle using motors in the calf. This can be modeled using our approach by having a serial model with 27 DoF along with 18 constrained DoF ($3 \times 6D$ contact constraints ).
This allows three internal mobility (the 3 rode in each closures can rotate freely).
Note that one can equivalently model the robot using 3D constraints, by replacing spherical joints in each closure by a 3D constraint.

\subsection{Kangaroo}
Kangaroo is the new humanoid robot of Pal Robotics, designed to have very high dynamic capabilities. As for Digit, the upper body of the robot is purely serial, and thus, only the lower body is modeled.
\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=0.32\textwidth]{Images/kangaroo.png}
         \caption{Kangaroo Robot}
         \label{fig:kangarooRobot}
     \end{subfigure}
     \hspace{0cm}
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=0.32\textwidth]{Images/kangaroo_modeled.png}
         \caption{Modeled kangaroo robot}
         \label{fig:kangarooModel}
     \end{subfigure}
    \caption{Real and modeled robot. The model is presented with open 6D and 3d contact constraint}
    \label{fig:kangaroo}
\end{figure}
The real and modeled robot are presented in figure \ref{fig:kangaroo}.
Kangaroo's leg has 6 linear actuators for 6 degrees of freedom. 
The robot is much more complex than the previous one as all the actuators are located in the hips, yield 12 kinematic closures.
We can again model the robot either using 3D or 6D constraints. 
In the model we provide, we used a mixture of three 6D constraints and nine 3D constraints, for a total of 45 constrained DoF.
The serial model has a total of 63 DoF, yielding 12 internal mobilities (the 12 rodes of the closures can rotate freely around their axis). 
